Signatured Deep Fictitious Play for Mean Field Games with Common Noise

Existing deep learning methods for solving mean-field games (MFGs) with common noise fix the sampling common noise paths and then solve the corresponding MFGs. This leads to a nested-loop structure with millions of simulations of common noise paths in order to produce accurate solutions, which results in prohibitive computational cost and limits the applications to a large extent. In this paper, based on the rough path theory, we propose a novel single-loop algorithm, named signatured deep fictitious play, by which we can work with the unfixed common noise setup to avoid the nested-loop structure and reduce the computational complexity significantly. The proposed algorithm can accurately capture the effect of common uncertainty changes on mean-field equilibria without further training of neural networks, as previously needed in the existing machine learning algorithms. The efficiency is supported by three applications, including linear-quadratic MFGs, mean-field portfolio game, and mean-field game of optimal consumption and investment. Overall, we provide a new point of view from the rough path theory to solve MFGs with common noise with significantly improved efficiency and an extensive range of applications. In addition, we report the first deep learning work to deal with extended MFGs (a mean-field interaction via both the states and controls) with common noise.

==> numerics.tex <==

In this section, we present the performance of Sig-DFP for three examples: homogeneous, heterogeneous and heterogeneous extended MFGs. A relative $L^2$ metric will be used for comparison, defined for progressively measurable random processes as
\begin{equation}
    L^2_R(x, \hat{x}) := \sqrt{\frac{\EE[\int_0^T \|x_t-\hat{x}_t\|^2\ud t]}{\EE[\int_0^T \|x_t\|^2\ud t]}}, \label{def: rela_L2}
\end{equation}
where $x$ is the true solution and $\hat{x}$ is the predicted result. We shall use stochastic gradient descent (SGD) optimizer for all three experiments.

{\bf Data preparation.} For all three experiments, the size of both training and testing data is  $N=2^{15}$, and the size of validation data is $N/2$. We fix $T=1$ and discretize $[0,1]$ by $t_{k}=\frac{k}{100},\; k=0,1,\dots,100$. Initial states are generated independently by $X_0^i \sim\mu_0$, with $\mu_0= U(0, 1)$ as the uniform distribution. The idiosyncratic Brownian motions $W$ and common noises $B$ are generated by antithetic sampling method, {\it i.e.}, we first generate half of the $(W^i, B^i)$ samples and get the other half by flipping them $(-W^i, -B^i)$.

%\subsection{Linear-Quadratic MFG}
{\bf Linear-Quadratic MFGs.} We first consider a Linear-Quadratic MFG with common noise proposed in \cite{carmona2015mean}, formulated as below:
\begin{align}
    & \inf_{\alpha_t} \EE\biggl\{\int_0^T \left[
    \frac{\alpha_t^2}{2}-q\alpha_t(m_t-X_t)+\frac{\epsilon}{2}(m_t-X_t)^2
    \right]\ud t \nonumber \\ & \hspace{5em}+\frac{c}{2}(m_T-X_T)^2 \biggr\}, \\
    &\text{subject to: }
    \ud X_t = [a(m_t-X_t)+\alpha_t]\ud t \nonumber\\& \hspace{7em} + \sigma(\rho \ud B_t + \sqrt{1-\rho^2}\ud W_t), \label{def:LQ_SDE}
\end{align}
where $m_t = \EE[X_t|\mcF^B_t]$ is the conditional mean, $\rho\in[0,1]$ is the noise correlation, and $q, \epsilon, c, a, \sigma$ are positive constants. We also assume $q\le \epsilon^2$ so that the cost function is jointly convex in state and control variables.

%\begin{align}
%    & \inf_{(\alpha_t)_{0\le t\le T}} \EE\left\{\int_0^T \left[
%    \frac{\alpha_t^2}{2}-q\alpha_t(m_t-X_t)+\frac{\epsilon}{2}(m_t-X_t)^2
%    \right]\ud t +\frac{c}{2}(m_T-X_T)^2 \right\}, \\
%    &\text{subject to: }
%    \ud X_t = [a(m_t-X_t)+\alpha_t]\ud t + \sigma(\rho \ud B_t + \sqrt{1-\rho^2}\ud W_t), \label{def:LQ_SDE}
%\end{align}

{\it Benchmark results} are provided by the analytical solution in \cite{carmona2015mean}:
\begin{align}
    & m_t = \EE[X_0] + \rho\sigma B_t, \quad t\in[0,T] \label{def:LQ_m} \\
    & \alpha_t^i = (q+\eta_t) (m_t -X_t^i), 
    \quad t\in[0,T], \label{def:LQ_alpha}
\end{align}
where $i$ represents the $i$-th player and 
$\eta_t = \frac{-(\epsilon-q^2)(e^{(\delta^+-\delta^-)(T-t)}-1) -c(\delta^+e^{(\delta^+-\delta^-)(T-t)}-\delta^-)}{(\delta^-e^{(\delta^+-\delta^-)(T-t)} \delta^+) -c(e^{(\delta^+-\delta^-)(T-t)} -1)}.$
Here $\delta^\pm = -(a+q)\pm \sqrt{R}$ and $R = (a+q)^2 + (\epsilon-q^2)>0$. The benchmark $X^i$ is simulated according to \eqref{def:LQ_SDE}  with $m_t$ and $\alpha_t^i$ in \eqref{def:LQ_m} and \eqref{def:LQ_alpha}.

 

{\it Training \& Results.} $\alpha_\varphi$ is estimated by a two hidden layers neural network with 64 hidden neurons in each layer. The signature depth for this example is $M=2$. Our model is trained over 500 rounds of fictitious play and the estimated $\hat{X}, \hat{\alpha}, \hat{m}$ are shown in Figure \ref{fig:LQ}. Note that fictitious play has a slow convergence speed due to that our initial guess $m^{(0)}$ is far from the truth. Therefore we only apply averaging over distributions (or linear functions) after the 250th iteration of fictitious play. We set learning rate as $0.1$ for the first half iterations and $0.01$ for the second half. The relative $L^2$ distances for testing data are listed in Table \ref{tab:LQ}.

\begin{table}[ht]
\caption{Relative $L^2$ errors on testing data for LQ-MFG.}
\label{tab:LQ}
\vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lcccr}
    \toprule
         &  SDE: $X_t$ & Control: $\alpha_t$ & Equilibrium: $m_t$\\
         \midrule
        $L^2_R$ & $0.0031$  & $0.0044$ & $0.058$ \\
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
\end{table}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{SystemicRisk/SDE.pdf}
         \caption{$X_t$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{SystemicRisk/alpha.pdf}
         \caption{$\alpha_t$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{SystemicRisk/mt.pdf}
         \caption{$m_t$}
     \end{subfigure}
    \caption{Plots on testing data for three different $(X_0^i, W^i, B^i)$. Solid line is the benchmark solution and dashed line is the predicted result. (a) Controlled SDE $X_t$; (b) Optimal control $\alpha_t$; (c) Conditional distribution flow $m_t$. Parameters are: $\sigma=0.2, q=1, a=1, \epsilon=1.5, \rho=0.2, c=1$.}
    \label{fig:LQ}
\end{figure}

{\bf Mean Field Portfolio Game.} 
\cite{lacker2018mean} considered an optimal portfolio management problem under competition and relative performance criteria under the mean field regime. More specifically, there are different agents who are characterized by their type vector (a random vector) $\zeta=(\xi, \delta, \theta, \mu, \nu, \sigma)$. All agents use exponential (CARA) utilities and their goal is to maximized expected payoff given by
\begin{equation}
    \sup_{(\pi_t)_{0\le t\le T}} \EE\left[ -\exp{\left(-\frac{1}{\delta}(X_T-\theta m_T) \right)} \right],
\end{equation}
where the dynamics are 
\begin{equation}
    \ud X_t = \pi_t(\mu \ud t + \nu \ud W_t + \sigma \ud B_t), \quad X_0=\xi.
\end{equation}

Here $m$ is the conditional distribution flow and $m_t:=\EE[X|\mcF^B_t]$.

{\it Benchmark.} Given type vector $\zeta=(\xi, \delta, \theta, \mu, \nu, \sigma)$, the benchmark solutions given in \cite{lacker2018mean} are listed below
\begin{align}
    & \pi^*_t = \delta\frac{\mu}{\sigma^2+\nu^2} + \theta\frac{\sigma}{\sigma^2+\nu^2}\frac{\phi}{1-\psi}, \\
    & m_t = \EE[\xi] +\EE[\mu \pi^*]t + \EE[\sigma \pi^*]B_t,
\end{align}
where $\phi=\EE[\delta\frac{\mu\sigma}{\sigma^2+\nu^2}]$ and $\psi = \EE[\theta\frac{\sigma^2}{\sigma^2+\nu^2}]$.

{\it Training \& Results.} We consider signature depth $M=2$ and use a fully connected neural network $\pi_\varphi$ with 4 hidden layers\footnote{Since different plays are charaterized by type vectors $\zeta$, $\pi_\varphi$ takes $(\zeta, t, X_t, m_t)$ as input. Hidden neurons in each layer are (64, 32, 32, 16).} to estimate $\pi$. We train our model with 500 rounds fictitious play. The learning rate starts at $0.1$ and is reduced 
by a factor of $5$ after every 200 rounds. The relative $L^2$ distances for testing data are listed in Table \ref{tab:Invest}. We plot $X$, $m$ and validation utilities in Figure \ref{fig:Invest}.

\begin{table}[ht]
\caption{Relative $L^2$ errors on testing data for MF Portfolio Game.}
\label{tab:Invest}
\vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lcccr}
    \toprule
         &  SDE: $X_t$ & Invest: $\pi_t$ & Equilibrium: $m_t$\\
         \midrule
        $L^2_R$ & $0.068$  & $0.035$ & $0.085$ \\
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
\end{table}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Invest/SDE.pdf}
         \caption{$X_t$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Invest/Xbar.pdf}
         \caption{$m_t$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Invest/valid_util.pdf}
         \caption{Utility}
     \end{subfigure}
    \caption{Plots on testing data for three different $(X_0^i, W^i, B^i, \zeta^i)$. Solid line is the benchmark solution and dashed line is the predicted result. (a) Controlled SDE $X_t$; (b) Conditional distribution flow $m_t:=\EE[X_t|\mcF^B_t]$; (c) Utilities of validation data over fictitious play rounds. Parameters are: $\delta \sim U(5, 5.5), \mu\sim U(0.25, 0.35), \nu\sim U(0.2, 0.4), \theta\sim U(0,1), \sigma\sim U(0.2, 0.4)$.}
    \label{fig:Invest}
\end{figure}

%\subsection{Mean Field Game of Optimal Consumption and Investment}
%\label{sec:InvestConsump}

{\bf Mean Field Game of Optimal Consumption and Investment.}
Our last example consider an extended mean field game case, which is propsoed by \cite{lacker2020many}. This is example is similar to the second one, expect for including consumption and adopting a power (CRRA) utility function. More specifically, each agent is characterized by the type vector $\zeta=(\xi, \delta, \theta, \mu, \nu, \sigma, \epsilon)$ the maximized expected utility is given by
%\begin{equation}
 %   \begin{aligned}
  %      \sup_{(\pi_t)_{0\le t\le T}, (c_t)_{0\le t\le T}} \EE\biggl[ 
   % &\int_0^T U(c_t X_t(\Gamma_t m_t)^{-\theta}; \delta)\ud t \\ &+ \epsilon U(X_T m^{-\theta}_T;\delta)
    %\biggr],     \end{aligned}
 %\label{def: InvestConsumpValue}
%\end{equation}
\begin{equation}
        \sup_{\pi_t, c_t} \EE\biggl[ 
    \int_0^T U(c_t X_t(\Gamma_t m_t)^{-\theta}; \delta)\ud t + \epsilon U(X_T m^{-\theta}_T;\delta)
    \biggr],     
 \label{def: InvestConsumpValue}
\end{equation}
where $U(x; \delta) = \left\{ \begin{array}{lc}
    \frac{1}{1-1/\delta}x^{1-1/\delta} & \text{if } \delta\ne 1 \\
    \log x & \text{if } \delta= 1
\end{array} \right.$ and the dynamics are 
\begin{equation}
    \ud X_t = \pi_t X_t(\mu \ud t + \nu \ud W_t + \sigma \ud B_t) - c_tX_t \ud t,  \label{def: InvestConsumpSDE}
\end{equation}
with $\quad X_t, c_t>0 \text{ and } X_0=\xi$.
$\Gamma_t = \exp\EE[\log c^*_t |\mcF^B_t]$ and $m_t = \exp\EE[\log X_t |\mcF^B_t]$ are the mean field interactions of consumption and wealth. We will use an equivalent expression of \eqref{def: InvestConsumpSDE} derived by It\^{o}'s formula to ensure the sign of $X_t$,
\begin{equation}
    \ud \log X_t = \pi_t (\mu \ud t + \nu \ud W_t + \sigma \ud B_t) - \frac{1}{2}  (2c_t + \pi^2_t\sigma^2 + \pi^2_t\nu^2 )\ud t, \label{def: InvestConsumplogSDE}
\end{equation}
with $X_t, c_t>0 \text{ and } X_0=\xi$.

{\it Benchmark.} We will only consider the case with $\delta\ne 1$. From \cite{lacker2020many}, the analytical solutions are given by
\begin{align}
    &\pi^*_t = \frac{\delta\mu}{\sigma^2+\nu^2} - \frac{\theta(\delta-1)\sigma}{\sigma^2+\nu^2}\frac{\phi}{1+\psi}=:\pi^*, \\
    &c^*_t = \left(\frac{1}{\beta} + (\frac{1}{\lambda}-\frac{1}{\beta})e^{-\beta(T-t)} \right)^{-1}, \label{def: InvestConsump c}
\end{align}
%where $\phi$, $\psi$, $\lambda$, $\beta$ are given in \cite{lacker2020many}. 
where 
\begin{align}
    &\phi = \EE\left[\frac{\delta\mu\sigma}{\sigma^2+\nu^2}\right], \quad 
    \psi = \EE\left[\frac{\theta(\delta-1)\sigma}{\sigma^2+\nu^2}\right],\quad
    \lambda = \epsilon^{-\delta}\,\left(e^{ \EE\left[\log(\epsilon^{-\delta})\right]}\right)^{-\frac{\theta(\delta-1)}{1+\EE\left[\theta(\delta-1)\right]}},\\
    &\beta = \theta(\delta-1)\frac{\EE\left[\delta\rho\right]}{1+\EE\left[\theta(\delta-1)\right]}-\delta\rho,
\end{align}
and 
\begin{align}
    \rho = \left(1-\ovd\right)\,&\left\{\frac{\delta}{2(\sigma^2+\nu^2)}\left(\mu-\sigma\frac{\phi}{1+\psi}\theta(1-\ovd)\right)^2
    +\frac{1}{2}\left(\frac{\phi}{1+\psi}\right)^2\theta^2\left(1-\ovd\right)\right.\nonumber\\
    &-\theta\EE\left[\frac{\delta\mu^2-\theta(\delta-1)\sigma\mu\frac{\phi}{1+\psi}}{\sigma^2+\nu^2}\right]
    +\left. \frac{\theta}{2}\EE\left[\frac{(\delta\mu-\theta(\delta-1)\sigma\frac{\phi}{1+\psi})^2}{\sigma^2+\nu^2}\right]\right\}.
\end{align}
    


It is straightforward that $c^*_t$ in \eqref{def: InvestConsump c} doesn't depend on common noises and hence $\Gamma$ admits a unique solution for all agents
\begin{equation}
    \Gamma_t = \exp \EE[\log c^*_t].
\end{equation}
By \eqref{def: InvestConsumplogSDE}, we can easily get 
$$
\EE[\log X_t|\mcF^B_t] = \EE[\xi]+ \EE[\pi^*\mu - \frac{1}{2}\pi^*(\sigma^2+\nu^2)] t - \int_0^t \EE[c^*_t] \ud t + \pi^* \sigma B_t,
$$
and $m_t = \exp \EE[\log X_t|\mcF^B_t]$.


The benchmark solution of \eqref{def: InvestConsumpValue} is given by $\EE[v(0, \xi, \EE[\xi])]$, with 
\begin{equation}
v(t,x,y) = \eps\left(1-\ovd\right)^{-1} x^{1-\ovd}y^{-\theta(1-\ovd)}f(t)
\end{equation}
and $f(t)$ is defined by
\begin{equation}
    f(t) = \exp\left\{\int_t^T \left(\rho + \ovd c_s^* + \EE[c_s^*]\left(1-\ovd\right)\theta\right) \ud s \right\}
\end{equation}

{\it Training \& Results.} 
In this example, we use signature depth $M=4$. The optimal controls $(\pi_t, c_t)_{0\le t\le 1}$ are estimated by two neural networks $\pi_\varphi$ and $c_\varphi$, each with 3 hidden layers.\footnote{Due the nature of heterogeneous extended MFG, both $\alpha_\varphi$ and $c_\varphi$ take $(\zeta_t, t, X_t, m_t, \Gamma_t)$ as input. Hidden neurons in each layer are (64,64,64).} Due to the extended mean field interaction term $\Gamma_t$, we will propagate 2 conditional distribution flows, i.e. 2 linear functionals $\Bar{l}^{(n)}, \Bar{l}_c^{(n)}$ during each round fictitious play. Instead of estimating $m_t, \Gamma_t$ directly, we estimate $\EE[\log X_t|\mcF^B_t], \EE[\log c^*_t|\mcF^B_t]$ by $\langle \Bar{l}^{(n)}, S^4(B_{0:t}) \rangle$, $\langle \Bar{l}_c^{(n)}, S^4(B_{0:t}) \rangle$ and then take exponential to get $m_t, \Gamma_t$. To ensure the non-negativity condition of $X_t$, we evolve $\log X_t$ according to \eqref{def: InvestConsumplogSDE} and then take exponential to get $X_t$. For optimal consumption, $c_\varphi$ is used to predicted $\log c_t$ and thus $\exp c_\varphi$ gives the predicted $c_t$. After 600 rounds fictitious play training, with learning rate 0.1 and decaying by factor of 5 for every 200 rounds, the relative $L^2$ distances for testing data are listed in Table \ref{tab:InvestConsump}. We show three example trajectories in Figure \ref{fig:InvestConsump}.



\begin{table}[ht]
\caption{Relative $L^2$ errors on testing data for Optimal Consumption and Investment MFG.}
\label{tab:InvestConsump}
\vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lccccr}
    \toprule
         &  Invest: $\pi_t$ & Consumption: $c_t$ & $m_t$ & $\Gamma_t$\\
         \midrule
        $L^2_R$ & $0.1126$  & $0.0614$ & $0.0279$  & $0.0121$ \\
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
\end{table}





\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{InvestConsumption/SDE.pdf}
         \caption{$X_t$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{InvestConsumption/Xbar.pdf}
         \caption{$m_t$}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{InvestConsumption/Gamma.pdf}
         \caption{$\Gamma_t$}
     \end{subfigure}
    \caption{Plots on testing data for three different $(X_0^i, W^i, B^i, \zeta^i)$. Solid line is the benchmark solution and dashed line is the predicted result. (a) Controlled SDE $X_t$; (b) Conditional distribution flow $m_t:=\exp\EE[\log X_t|\mcF^B_t]$; (c) Conditional distribution flow $\Gamma_t:= \exp\EE[\log c^*_t |\mcF^B_t]$. Parameters are: $\delta \sim U(2, 2.5), \mu\sim U(0.25, 0.35), \nu\sim U(0.2, 0.4), \theta\sim U(0,1), \sigma\sim U(0.2, 0.4)$, $\epsilon\sim U(0.5, 1)$.}
    \label{fig:InvestConsump}
\end{figure}
